DT*: Temporal Logic Path Planning in a Dynamic Environment

Path planning for a robot is one of the major problems in the area of robotics. When a robot is given a task in the form of a Linear Temporal Logic (LTL) specification such that the task needs to be carried out repetitively, we want the robot to follow the shortest cyclic path so that the number of times the robot completes the mission within a given duration gets maximized. In this paper, we address the LTL path planning problem in a dynamic environment where the newly arrived dynamic obstacles may invalidate some of the available paths at any arbitrary point in time. We present DT*, an SMT-based receding horizon planning strategy that solves an optimization problem repetitively based on the current status of the workspace to lead the robot to follow the best available path in the current situation. We implement our algorithm using the Z3 SMT solver and evaluate it extensively on an LTL specification capturing a pick-and-drop application in a warehouse environment. We compare our SMT-based algorithm with two carefully crafted greedy algorithms. Our experimental results show that the proposed algorithm can deal with the dynamism in the workspace in LTL path planning effectively.

==> old_describtion.tex <==
Algorithm 1 outlines the major steps in our approach. Given a workspace $W$ modelled by $T$ and an LTL query $\phi$, we want to generate dynamic plans for the robot so that the robot can deal with the changes in the environment.
For the generation of the reduced graph $G_r$, we use a procedure given in~\cite{Tstar}, denoted by $gen\_redc\_graph()$ on line~\ref{line2}. 

% In the initial static environment, we generate a plan using the method $\mathtt{plan\_in\_H()}$ with static edge costs of edges in $G_r$, the initial
In the initial static environment, we generate a plan of the form $R = prefix.{suffix}^\omega$ on line~\ref{line4}, where $prefix$ is the path from the initial location to a destination location $d \in F_r$, such that the cycle $suffix$ from $d$ is the minimum length cycle. This $suffix$ is repeated perpetually if the environment does not change. 

The robot keeps traversing this infinite path $R$ until some changes in the workspace are observed or the plan gets empty. 
% Firstly, we'll add the current position, as a new node in $G_r$ and then generate each edge's cost within horizon starting from $time_{cur}$.

Firstly, we make the changes in the transition system depending upon the changes in workspace $W$, if any.
Then, we pre-compute all the edge costs of $G_r$ within horizon $H$. Procedure $dy\_cost()$ on line~\ref{line14} is similar to the one given in \cite{llastar}.
We call the time taken for computing all the edge costs of $G_r$ within $H$ as pre-computation time.

\noindent
The ${plan\_in\_H()}$ procedure which is invoked on line~\ref{line15}, is the planning in horizon method, with all the pre-computed edge costs as one of the parameter. The procedure $plan\_in\_H()$ firstly generates the constraints for modeling the decision problem for the robot from the current timestamp using procedure $gen\_{cons}()$ on line~\ref{line17}. The upperbound on the sum of the time taken by the SMT solver to solve the constraint based model and the pre-computation time is referred to as $time_{comp}$.  

\noindent
The $plan\_in\_H()$ procedure returns the optimal decision sequence, within the given horizon $H$ from the current robot position $pos_{cur}$ for the robot, if one exists.
If it does not, then we use the same $plan\_in\_H()$ procedure again, until we get some optimal decision sequence. While doing so we'll update $time_{cur}$ based on the total computation time $time_{comp}$ taken the SMT solver based approach. Procedure $get\_plan\_from\_model()$ on line~\ref{line20}, simply parses the model solution to get path within $H$ from optimal decision sequence.
 
\noindent
\textbf{Example.}
Figure~\ref{fig4} shows the application of our algorithm on example that we have discussed earlier in Figure~\ref{fig1}. Figure~\ref{fig4}a, shows the reduced product graph $G_r$ in the initial static environment. When the environment changes at timestamp 10, we add a node in the previous graph $G_r$ based on the current robot position and it's B\"{u}chi state, as shown in Figure~\ref{fig4} b. We pass the environment changes observed, the updated product graph along with other parameters to a procedure $dy\_cost()$. The pre-computated edge costs within $H$ will be later used by constraint generation procedure. It was found empirically that having this precomputation step is better than calling $A^*$ multiple times while model creation.

\noindent
Constraint generation is done by $gen\_cons()$ procedure and will be discussed in the next section.







To understand the problem better, let us consider an example.
Figure~\ref{fig1.1} shows the B\"uchi automaton for the LTL specification that captures a warehouse scenario where the robot is given a task which needs to be repeated forever: \textit{The robot should pick up an object from some location and drop it to some other designated location. Once an object is picked up, the robot cannot go to a pickup location again until it goes to some drop location, and once an object is dropped , robot cannot go to a drop location until it goes to some pickup location.}

Figure~\ref{fig1.2} shows a sample workspace with 3 pickup and 3 drop locations marked as $P1$, $P2$, $P3$ and $D1$, $D2$, $D3$, respectively. 
As shown in Figure~\ref{fig1.2}, the initial solution generated by $Greedy_1$ algorithm is prefix path $\langle(0,0), (6,2), (7,0) \rangle$ shown in blue followed by the minimum length suffix cycle $\langle (7,0),(6,2),(7,0)\rangle$ marked in red from drop location $D3$.
Another solution which is generated by $Greedy_2$ algorithm is shown with green prefix path $\langle (0,0),(1,2),(1,7)\rangle$ till location $D1$ followed by the suffix cycle $\langle ((1,7)(1,2),(1,7) \rangle$ of length $10$ starting at $D1$.
Suppose that both paths are getting traversed by some robot. At timestamp $10$, some proposition locations becomes unavailable as shown in Figure~\ref{fig1.3}. The current robot position for both the paths generated by $Greedy_1$ and $Greedy_2$ algorithm is shown through blue and green dots respectively. Now, both $Greedy_1$ and $Greedy_2$ algorithm replans based on the current workspace condition. 
$Greedy_1$ algorithm considers cycle $\langle (6,8),(8,5),(6,8)\rangle$ as the minimum length cycle. 
Thus, the robot starts traversing a prefix to reach $(6,8)$. But at $Ts = 20$, $P3$ becomes available again, $Greedy_1$ then replans at $Ts=20$ with prefix from $(5,7)$ to $(7,0)$ till $Ts=31$. 
Then, covering suffix cycles of length 8 from $D3$ at Ts=39 and 47 respectively. Overall, $Greedy_1$ covers 2 suffix cycles upto $ts=47$. 
$Greedy_2$ algorithm minimizes the overall time to complete $prefix+suffix$. From $(1,5)$ it goes to $(8,5)$ and then at $(7,0)$ at Ts=23. It then, completes the first suffix cycle at $Ts=31$. Upto $Ts=47$, $Greedy_2$ algorithm covers a total of 3 suffix cycles.

We can see the difference in the number of cycles generated by $Greedy_1$ and $Greedy_2$ algorithms based on the decisions taken. However, there exists a better plan which could complete even more cycles within the same duration.
Consider, the robot location to be blue dot (same as $Greedy_1$) algorithm at Ts=10. Now, the decision could be to traverse a longer cycle of length 12, considering the fact that $P3$ will become available at Ts=20. So ,the robot moves from $(7,1)$ to $(7,0)$ at $Ts=11$. 
Then, it completes a cycle $\langle (7,0),(8,5),(7,0)\rangle$ till $Ts=23$. 
Now, a cycle of length $8$ exists from location $D3$. The robot then completes cycles at Ts=31, 39 and 47 respectively, thereby covering a total of 4 cycles upto Ts=47. The timelines for all the discussed solutions for sample environment in shown in Figure~\ref{fig2}.

The decision to be made by the robot is to choose whether to switch to another cycle, to repair the current trajectory or to simply wait for the proposition locations to become available again.
In this paper we attempt to solve this problem by reducing it to an optimization problem, where we model the above decision problem for a single robot as a \textit{constraint satisfaction problem} and feed it to an SMT solver with the objective function to maximize the number of times the task is completed within a finite horizon $H$.


% As shown in \textit{Fig.2}, suppose the robot starts traversing the path from timestamp 0 and reaches $(0,1)$ .\textit{Fig.3} shows that the robot is at location $(0,1)$ at timestamp 1, when some changes in the environment are observed.\\
% As shown in \textit{Fig.3}, proposition locations  $(4,8),(7,0)$ are unreachable till timestamps 36 and 11 respectively.\\
% In the current environment the greedy strategy, which is greedy about shortest available loop in current workspace will follow the cycle,$(2,0)(7,0)(2,0)$\textit{(shown in blue)}. As shown in \textit{Fig. 3.2}, at timestamp 36, when a shorter suffix cycle becomes available, the robot switches to the smaller cycle $(4,5)(4,8)(4,5)$\textit{(shown in blue)}.\\
% Till timestamp 51, the total number of cycles that could be covered by the robot using greedy strategy are 2, which is not optimal and the robot could have covered more suffix cycles within same time.\\
% \textit{Fig.3.3} shows an better plan, which could complete more number of cycles by taking appropriate decisions.
% As shown in \textit{Fig.3.3}, the first decision to switch to a longer cycle $(4,5)(9,3)(4,5)$,\textit{(shown in blue)} as one shorter cycle will become available again $(4,5)(4,8)(4,5)$\textit{(shown in pink)}.In total the above decision sequence results in completion of 3 suffix cycles till timestamp 51.
% The gain in terms of number of suffix cycles traversed till timestamp 51 is of 1 cycle.
